Cheetah: Natural Language Generation for 517 African Languages

Low-resource African languages pose unique challenges for natural language processing (NLP) tasks, including natural language generation (NLG). In this paper, we develop Cheetah, a massively multilingual NLG language model for African languages. Cheetah supports 517 African languages and language varieties, allowing us to address the scarcity of NLG resources and provide a solution to foster linguistic diversity. We demonstrate the effectiveness of Cheetah through comprehensive evaluations across six generation downstream tasks. In five of the six tasks, Cheetah significantly outperforms other models, showcasing its remarkable performance for generating coherent and contextually appropriate text in a wide range of African languages. We additionally conduct a detailed human evaluation to delve deeper into the linguistic capabilities of Cheetah. The introduction of Cheetah has far-reaching benefits for linguistic diversity. By leveraging pretrained models and adapting them to specific languages, our approach facilitates the development of practical NLG applications for African communities. The findings of this study contribute to advancing NLP research in low-resource settings, enabling greater accessibility and inclusion for African languages in a rapidly expanding digital landscape. We publicly release our models for research.

==> tables/datasetinfo.tex <==
\begin{table*}[hbt!]
\centering
\scriptsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{c}{}                                 & \multicolumn{2}{c}{\textbf{Vocabulary}}                                    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}    & \multicolumn{3}{c}{\textbf{Training Data}}                                                                          \\\cline{2-3}   \cline{6-8} 
\multicolumn{1}{l}{\multirow{-2}{*}{\textbf{Model}}} & \multicolumn{1}{c}{\textbf{Tok}} & \multicolumn{1}{c}{\textbf{Vocab Size}} & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{\#Params}}}      & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{\#Lang.} (afr/all)}} & \multicolumn{1}{c}{\textbf{Tokens} (afr/all)} & \multicolumn{1}{c}{\textbf{Size} (afr/all)} & \multicolumn{1}{c}{\textbf{Source}} \\
\midrule
ourmodel-E250                                       & WP                               & 250K                                    & 277M                                        & 517/527                                      & 7.1B/8.6B                                &40/42GB                              & RT, News, GD, HD, EC                                        \\
\ourmodelnlg                                            & SP                               & 250K                                    & 278M                                         & 517/527                                     & 7.1B/8.6B                                &40/42GB		                               & RT, News, GD, HD, EC   \\ \bottomrule
\end{tabular}
}
\caption{Models with African languages that we compare our model with. SP: SentencePiece, WP: WordPiece. Data sources include - CC: CommonCrawl, EC: Existing corpora, GD: Government documents, HD: Health documents, RT: Religious text, UNK: Unknown.}
\label{tab:encoder-only}
\end{table*}

==> tables/mt_results.tex <==
\begin{table*}[hbt!]
\scriptsize
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llllll}
\toprule
\textbf{Task\_id}  & \textbf{mT0-base} & \textbf{mt5-base} & \textbf{Afriteva\_base} & \textbf{\ourmodelnlg} \\ \toprule
 mt-afroMT-eng-afr               & \textbf{20.03}                 &7.94                 & 3.53                       & \textbf{26.68}                        \\
 mt-afroMT-eng-bem               & 19.19             & 12.88             & \textbf{27.49}          & 18.6                      \\
                                   % & mt-afroMT-eng-lin               & \textbf{14.90}                 & \textbf{11.90}                 & \textbf{6.96}                       & \textbf{9.68}                         \\
 mt-afroMT-eng-run               & \textbf{14.9}     & 11.9              & 6.96                    & 9.68                      \\
                                   % & mt-afroMT-eng-sot               & 0                 & 0                 & 0                       & 0                         \\
 mt-afroMT-eng-swa               & 6.06                 & 7.43                 & 4.05                       & \textbf{8.34}                         \\
 mt-afroMT-eng-xho               & 11.7                & 12.43                 & 6.04                       & \textbf{13.54}                         \\
 mt-afroMT-eng-zul               & 7.07                 & 6.12                 & 7.09                      & \textbf{8.01}                        \\
 mt-lafand-eng-hau               & 10.32             & 8.63              & 7.72                    & \textbf{12.87}            \\
 mt-lafand-eng-ibo               & 17.72             & 17.31             & 13.71                   & \textbf{19.66}            \\
 mt-lafand-eng-lug               & 8.2               & 7.1               & 4.85                    & \textbf{11.42}            \\
 mt-lafand-eng-pcm               & \textbf{33.49}    & 33.09             & 30.07                   & 33.43                     \\
                                   % & mt-lafand-eng-swa               & 0                 & 0                 & 0                       & 0                         \\
 mt-lafand-eng-tsn               & 11.93             & 10.16             & \textbf{19.44}                    & \textbf{19.44}            \\
 mt-lafand-eng-twi               & 5.19              & 3.69              & 2.12                    & \textbf{6.63 }                     \\
 mt-lafand-eng-yor               & 8.3               & 7.57              & 5.81                    & \textbf{10.13}            \\
 mt-lafand-eng-zul               & 12.3              & 1.6                & 9.35                    & \textbf{14.75}            \\
 mt-lafand-fra-bam               & 9.53              & 4.56              & 5.29                    & \textbf{9.67}             \\
 mt-lafand-fra-bbj               & 1.36              & 1.11              & 1.02                    & \textbf{1.73}             \\
 mt-lafand-fra-ewe               & 3.29              & 1.93              & 1.02                    & \textbf{4.63}             \\
 mt-lafand-fra-fon               & 2.51              & 0.71              & 2.06                    &\textbf{ 4.4 }                      \\
 mt-lafand-fra-mos               & 0.51              & 0.48              & 0.32                    & \textbf{1.66}             \\
 mt-lafand-fra-wol               & \textbf{6.91}     & 4.39              & 3.98                    & 6.16                      \\
 mt-pidginUNMT-eng-pcm           & 30.63             & 30.72             & 24.78                   & \textbf{31.53}            \\
 mt-salt-ach-eng                 & 20.98                 & 19.47                 & 20.23                       & 22.43   \\
 mt-salt-ach-lgg                 & 6.83               & 7.87                 & 8.91                       & \textbf{11.42}                         \\
 mt-salt-ach-lug                 & 5.32                & 4.15                 & 6.44                       & \textbf{11.17}                         \\
 mt-salt-ach-nyn                 & 4.32                & 3.36                 & 4.70                       & \textbf{7.36}                         \\
 mt-salt-ach-teo                 & 6.88                 & 5.56                 & 9.1                       &\textbf{11.17}                         \\
 mt-salt-eng-lgg                 &15.87                 & 15.15                 & 12.59                      & 16.15                         \\
 mt-salt-eng-lug                 & 17.93                 & 18.76                 & 14.76                      & \textbf{21.97}                         \\
 mt-salt-eng-nyn                 & 10.49                 & 9.99                 & 10.12                       & \textbf{12.21}                        \\
 mt-salt-eng-teo                 & 16.33                 & 15.78                & 14.00                       & \textbf{16.98}                         \\
 mt-salt-lgg-teo                 & 5.17                & 4.24                 & 7.45                       & 8.85                         \\
 mt-salt-lug-lgg                 & 8.49                 & 7.43                 & 8.84                       & \textbf{12.17}                         \\
 mt-salt-lug-teo                 & 9.3                 & 8.22                 & 9.22                       & \textbf{12.73}                         \\
 mt-salt-nyn-lgg                 & 7.14                 & 5.69                 & 7.32                       & \textbf{10.95}                        \\
 mt-salt-nyn-lug                 &7.87                 & 5.32                 & 11.05                       & 15.81                         \\
 mt-salt-nyn-teo                 & 6.91                 & 5.33                 & 7.78                       & \textbf{10.3}                         \\ \hline
MT Score & 10.86 & 9.24 & 9.04 & \textbf{12.76} \\\bottomrule
\end{tabular}
}
\caption{Results on MT}
\label{tab:mtresults}
\end{table*}
         

==> tables/results_with_afri-mt5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!]
\scriptsize
\centering
\begin{tabular}{llllllll} \toprule
\textbf{Cluster}                            & \textbf{Task}                                              & \textbf{Metric} & \textbf{mT0}        &\textbf{ mT5}        & \textbf{Afri-MT5}    & \textbf{AfriTeVa}     & \textbf{Cheetah}        \\ \toprule
\multirow{39}{*}{\rotatebox[origin=]{90}{\textbf{Machine Translation (MT)}}}                & English $\rightarrow$ Afrikaans                    & Bleu   & 20.38\textsuperscript{$\pm$0.3 }  & 12.35\textsuperscript{$\pm$1.1 }  & 7.12\textsuperscript{$\pm$2.67 }   & 7.75\textsuperscript{$\pm$1.67}    & 19.72\textsuperscript{$\pm$0.75}     \\
                                   & English $\rightarrow$ Bemba                        & Bleu   & 19.19\textsuperscript{$\pm$0.3 }  & 12.28\textsuperscript{$\pm$0.48 } & 11.73\textsuperscript{$\pm$12.3 }  & 20.5\textsuperscript{$\pm$0.87 }    & 18.9\textsuperscript{$\pm$1.22 }     \\
                                   & English $\rightarrow$ Lingala                      & Bleu   & 15.98\textsuperscript{$\pm$1.16 } & 14.12\textsuperscript{$\pm$0.56 } & 14.32\textsuperscript{$\pm$12.74 } & 13.88\textsuperscript{$\pm$1.04 }   & 9.64\textsuperscript{$\pm$1.11}      \\
                                   & English $\rightarrow$ Rundi                        & Bleu   & 12.26\textsuperscript{$\pm$0.47 } & 8.82\textsuperscript{$\pm$0.43 }  & 9.57\textsuperscript{$\pm$0.42 }   & 7.83\textsuperscript{$\pm$1.04 }    & 10.54\textsuperscript{$\pm$0.54 }     \\
                                   & English $\rightarrow$ Sesotho                      & Bleu   & 11.04\textsuperscript{$\pm$1.2 }  & 12.74\textsuperscript{$\pm$0.75 } & 10.0\textsuperscript{$\pm$1.79 }  & 10.76\textsuperscript{$\pm$1.4 }    & 13.3\textsuperscript{$\pm$1.38 }      \\
                                   & English $\rightarrow$ Swahili                      & Bleu   & 10.59\textsuperscript{$\pm$1.84 } & 9.33\textsuperscript{$\pm$0.58 }  & 3.08\textsuperscript{$\pm$0.57 }   & 7.24\textsuperscript{$\pm$0.46 }    & 11.08\textsuperscript{$\pm$0.61}     \\
                                   & English $\rightarrow$ Xhosa                        & Bleu   & 10.04\textsuperscript{$\pm$0.98 } & 8.25\textsuperscript{$\pm$0.7 }   & 3.86\textsuperscript{$\pm$1.35 }   & 7.5\textsuperscript{$\pm$0.32 }     & 12.34\textsuperscript{$\pm$0.51 }     \\
                                   & English $\rightarrow$ Zulu                         & Bleu   & 17.65\textsuperscript{$\pm$1.86 } & 17.97\textsuperscript{$\pm$1.69 } & 1.9\textsuperscript{$\pm$1.11 }    & 13.45\textsuperscript{$\pm$1.81 }   & 19.49\textsuperscript{$\pm$1.16 }     \\
                                   & English $\rightarrow$ Hausa                        & Bleu   & 5.06\textsuperscript{$\pm$0.21 }  & 4.96\textsuperscript{$\pm$0.16 }  & 0.85\textsuperscript{$\pm$0.04 }   & 7.32\textsuperscript{$\pm$0.00 }     & 9.22\textsuperscript{$\pm$0.08 }     \\
                                   & English $\rightarrow$ Igbo                         & Bleu   & 13.05\textsuperscript{$\pm$0.17 } & 11.57\textsuperscript{$\pm$0.23 } & 1.12\textsuperscript{$\pm$0.09 }   & 12.34\textsuperscript{$\pm$0.23 }   & 16.75\textsuperscript{$\pm$0.26 }     \\
                                   & English $\rightarrow$ Luganda                      & Bleu   & 2.17\textsuperscript{$\pm$2.77 }  & 3.33\textsuperscript{$\pm$0.35 }  & 0.09\textsuperscript{$\pm$0.01 }   & 4.21\textsuperscript{$\pm$0.77 }    & 9.75\textsuperscript{$\pm$0.01 }      \\
                                   & English $\rightarrow$ Nigerian Pidgin              & Bleu   & 33.17\textsuperscript{$\pm$0.28 } & 32.65\textsuperscript{$\pm$0.19 } & 2.39\textsuperscript{$\pm$0.23 }   & 9.39\textsuperscript{$\pm$0.18}    & 32.64\textsuperscript{$\pm$0.14 }     \\
                                   & English $\rightarrow$ Swahili                      & Bleu   & 22.04\textsuperscript{$\pm$2.89 } & 23.2\textsuperscript{$\pm$0.23 }  & 2.79\textsuperscript{$\pm$0.08 }   & 22.39\textsuperscript{$\pm$0.28 }   & 28.11\textsuperscript{$\pm$0.14 }     \\
                                   & English $\rightarrow$ Zulu                         & Bleu   & 6.83\textsuperscript{$\pm$0.29}  & 0.58\textsuperscript{$\pm$1.37 }  & 0.4\textsuperscript{$\pm$0.03 }    & 4.45\textsuperscript{$\pm$0.37 }    & 11.75\textsuperscript{$\pm$0.38 }     \\
                                   & English $\rightarrow$ Twi                          & Bleu   & 3.4\textsuperscript{$\pm$0.12 }   & 1.23\textsuperscript{$\pm$0.03}  & 0.03\textsuperscript{$\pm$0.0}   & 1.68\textsuperscript{$\pm$0.94 }    & 4.64\textsuperscript{$\pm$0.13 }      \\
                                   & English $\rightarrow$ Yoruba                       & Bleu   & 5.42\textsuperscript{$\pm$0.85 }  & 2.58\textsuperscript{$\pm$3.1 }   & 0.04\textsuperscript{$\pm$0.0}    & 3.63\textsuperscript{$\pm$4.01 }    & 7.83\textsuperscript{$\pm$0.14 }      \\
                                   & English $\rightarrow$ Zulu                         & Bleu   & 10.28\textsuperscript{$\pm$0.49 } & 1.31\textsuperscript{$\pm$2.26 }  & 0.14\textsuperscript{$\pm$0.03 }   & 3.8\textsuperscript{$\pm$4.2 }     & 12.13\textsuperscript{$\pm$0.1 }      \\
                                   & French $\rightarrow$ Bambara                       & Bleu   & 2.0\textsuperscript{$\pm$2.6 }    & 0.37\textsuperscript{$\pm$0.19 }  & 0.15\textsuperscript{$\pm$0.01 }   & 3.18\textsuperscript{$\pm$0.18 }    & 3.06\textsuperscript{$\pm$0.27 }      \\
                                   & French $\rightarrow$ Ghomálá’                      & Bleu   & 0.4\textsuperscript{$\pm$0.09 }   & 0.33\textsuperscript{$\pm$0.01 }  & 0.07\textsuperscript{$\pm$0.0}    & 0.96\textsuperscript{$\pm$0.01 }    & 0.28\textsuperscript{$\pm$0.25 }     \\
                                   & French $\rightarrow$ Ewe                           & Bleu   & 0.7\textsuperscript{$\pm$0.35 }   & 0.31\textsuperscript{$\pm$0.36 }  & 0.09\textsuperscript{$\pm$0.07 }   & 0.84\textsuperscript{$\pm$0.16 }    & 3.47\textsuperscript{$\pm$0.03 }      \\
                                   & French $\rightarrow$ Fon                           & Bleu   & 0.69\textsuperscript{$\pm$0.31 }  & 0.8\textsuperscript{$\pm$0.13 }  & 1.52\textsuperscript{$\pm$0.06 }   & 1.73\textsuperscript{$\pm$0.53}    & 1.29\textsuperscript{$\pm$0.16 }      \\
                                   & French $\rightarrow$ Moore                         & Bleu   & 0.27\textsuperscript{$\pm$0.06 }  & 0.12\textsuperscript{$\pm$0.05 }  & 0.19\textsuperscript{$\pm$0.02}   & 0.47\textsuperscript{$\pm$0.04 }    & 1.66\textsuperscript{$\pm$0.86 }      \\
                                   & French $\rightarrow$ Wolof                         & Bleu   & 4.02\textsuperscript{$\pm$0.12 }  & 0.3\textsuperscript{$\pm$0.05 }   & 0.11\textsuperscript{$\pm$0.01}   & 3.08\textsuperscript{$\pm$0.25 }    & 3.01\textsuperscript{$\pm$0.07 }     \\
                                   & English $\rightarrow$ Nigerian Pidgin (pidginUNMT) & Bleu   & 27.44\textsuperscript{$\pm$0.26 } & 23.42\textsuperscript{$\pm$1.61 } & 7.05\textsuperscript{$\pm$1.37 }   & 22.54\textsuperscript{$\pm$0.84 }   & 26.56\textsuperscript{$\pm$0.04 }      \\
                                   & Acholi $\rightarrow$ English                       & Bleu   & 16.41\textsuperscript{$\pm$0.08 } & 11.16\textsuperscript{$\pm$4.77 } & 4.9\textsuperscript{$\pm$0.11 }    & 8.37\textsuperscript{$\pm$8.12 }    & 19.33\textsuperscript{$\pm$0.1 }      \\
                                   & Acholi $\rightarrow$ Lugbara                       & Bleu   & 2.57\textsuperscript{$\pm$0.21 }  & 1.48\textsuperscript{$\pm$1.31 }  & 2.44\textsuperscript{$\pm$0.37 }   & 8.29\textsuperscript{$\pm$0.14 }    & 7.21\textsuperscript{$\pm$0.69 }      \\
                                   & Acholi $\rightarrow$ Luganda                       & Bleu   & 3.64\textsuperscript{$\pm$0.07 }  & 1.74\textsuperscript{$\pm$0.12 }  & 0.92\textsuperscript{$\pm$0.01 }   & 5.53\textsuperscript{$\pm$0.34 }    & 8.03\textsuperscript{$\pm$0.38 }      \\
                                   & Acholi $\rightarrow$ Nyankore                      & Bleu   & 2.17\textsuperscript{$\pm$0.14 }  & 0.79\textsuperscript{$\pm$0.51 }  & 0.46\textsuperscript{$\pm$0.03 }   & 4.26\textsuperscript{$\pm$0.54 }    & 5.1\textsuperscript{$\pm$0.14 }  \\
                                   & Acholi $\rightarrow$ Ateso                         & Bleu   & 1.64\textsuperscript{$\pm$2.34 }  & 1.94\textsuperscript{$\pm$0.25}  & 4.9\textsuperscript{$\pm$0.11 }    & 7.74\textsuperscript{$\pm$0.33 }    & 6.33\textsuperscript{$\pm$0.6 }       \\
                                   & English $\rightarrow$ Lugbara                      & Bleu   & 6.19\textsuperscript{$\pm$6.33 }  & 8.38\textsuperscript{$\pm$0.49 }  & 5.93\textsuperscript{$\pm$0.22 }   & 10.95\textsuperscript{$\pm$0.32 }   & 11.61\textsuperscript{$\pm$0.28 }     \\
                                   & English $\rightarrow$ Luganda                      & Bleu   & 12.08\textsuperscript{$\pm$0.03 } & 10.58\textsuperscript{$\pm$0.25 } & 2.59\textsuperscript{$\pm$0.73 }   & 12.41\textsuperscript{$\pm$0.35 }   & 17.12\textsuperscript{$\pm$0.16 }    \\
                                   & English $\rightarrow$ Nyankore                     & Bleu   & 6.46\textsuperscript{$\pm$0.08 }  & 5.69\textsuperscript{$\pm$0.02 }  & 1.4\textsuperscript{$\pm$0.39 }    & 7.88\textsuperscript{$\pm$0.18 }    & 9.04\textsuperscript{$\pm$0.24 }      \\
                                   & English $\rightarrow$ Ateso (salt)                 & Bleu   & 10.24\textsuperscript{$\pm$0.06 } & 8.28\textsuperscript{$\pm$0.19 }  & 4.91\textsuperscript{$\pm$0.59 }   & 11.64\textsuperscript{$\pm$0.49 }   & 11.12\textsuperscript{$\pm$0.38 }     \\
                                   & Lugbara $\rightarrow$ Ateso                        & Bleu   & 2.21\textsuperscript{$\pm$0.35 }  & 1.5\textsuperscript{$\pm$0.2 }    & 2.22\textsuperscript{$\pm$0.15 }   & 6.67\textsuperscript{$\pm$0.32 }    & 3.68\textsuperscript{$\pm$0.31 }      \\
                                   & Luganda $\rightarrow$ Lugbara                      & Bleu   & 3.96\textsuperscript{$\pm$0.57 }  & 2.61\textsuperscript{$\pm$0.12 }  & 3.44\textsuperscript{$\pm$0.32 }   & 8.05\textsuperscript{$\pm$0.23 }    & 7.99\textsuperscript{$\pm$0.47 }      \\
                                   & Luganda $\rightarrow$ Ateso                        & Bleu   & 4.47\textsuperscript{$\pm$0.08 }  & 3.01\textsuperscript{$\pm$0.16 }  & 2.5\textsuperscript{$\pm$0.22 }    & 8.17\textsuperscript{$\pm$0.18 }    & 8.13\textsuperscript{$\pm$0.33 }      \\
                                   & Nyankore $\rightarrow$ Lugbara                     & Bleu   & 3.45\textsuperscript{$\pm$0.29 }  & 2.1\textsuperscript{$\pm$0.32 }   & 2.6\textsuperscript{$\pm$0.29 }    & 7.5\textsuperscript{$\pm$0.09 }     & 7.29\textsuperscript{$\pm$0.09 }     \\
                                   & Nyankore $\rightarrow$ Luganda                     & Bleu   & 8.54\textsuperscript{$\pm$0.17 }  & 6.91\textsuperscript{$\pm$0.23 }  & 2.01\textsuperscript{$\pm$0.25 }   & 6.77\textsuperscript{$\pm$6.73 }    & 6.25\textsuperscript{$\pm$10.26 }     \\
                                   & Nyankore $\rightarrow$ Ateso                       & Bleu   & 3.33\textsuperscript{$\pm$0.11 }  & 2.25\textsuperscript{$\pm$0.23 }  & 2.12\textsuperscript{$\pm$0.4 }    & 6.27\textsuperscript{$\pm$0.12 }    & 6.36\textsuperscript{$\pm$0.4 }      \\ \midrule
\multirow{3}{*}{\textbf{Paraphrase}}       &  Multilingual                           & Bleu   & 41.79\textsuperscript{$\pm$0.28 } & 41.75\textsuperscript{$\pm$0.21 } & 34.72\textsuperscript{$\pm$0.51 }  & 43.02\textsuperscript{$\pm$1.25 }  & 43.23\textsuperscript{$\pm$0.09 }     \\
                                   &  Berber                                 & Bleu   & 44.84\textsuperscript{$\pm$0.31 } & 44.03\textsuperscript{$\pm$0.24 } & 36.08\textsuperscript{$\pm$0.83}  & **46.41\textsuperscript{$\pm$0.71 } & 46.0\textsuperscript{$\pm$0.27 }      \\
                                   &  Kabyle                                 & Bleu   & 25.91\textsuperscript{$\pm$0.13 } & 25.32\textsuperscript{$\pm$0.46 } & 11.56\textsuperscript{$\pm$0.73}  & 16.06\textsuperscript{$\pm$14.79 }  & 26.27\textsuperscript{$\pm$0.56 }     \\ \midrule
{\textbf{Question Answering}}                 & QA Swahili                                       & F1     & 79.84\textsuperscript{$\pm$0.19 } & 72.04\textsuperscript{$\pm$0.54 } & 0           & 62.64\textsuperscript{$\pm$0.78 }   & 71.98\textsuperscript{$\pm$1.18 }    \\ \midrule
 % \multirow{11}{*}{\rotatebox[origin=]{90}{\multicolumn{1}{c}{\textbf{Summarization}} }} 
\multirow{11}{*}{\rotatebox[origin=]{90}{\textbf{Summarization}}}    &  Multilingual                            & RougeL & 22.31\textsuperscript{$\pm$0.12 } & 22.23\textsuperscript{$\pm$0.04 } & 5.34\textsuperscript{$\pm$0.48 }     & 18.97\textsuperscript{$\pm$0.06 }   & 24.86\textsuperscript{$\pm$0.02 }     \\
                                   &  Amharic                                 & RougeL & 13.81\textsuperscript{$\pm$0.04 } & 13.09\textsuperscript{$\pm$0.03 } & 4.4\textsuperscript{$\pm$1.07}    & 8.29\textsuperscript{$\pm$0.51 }    & 15.09\textsuperscript{$\pm$0.1 }      \\
                                   &  Igbo                                    & RougeL & 18.9\textsuperscript{$\pm$0.73 }  & 13.22\textsuperscript{$\pm$0.46 } & 14.24\textsuperscript{$\pm$0.39 }  & 16.05\textsuperscript{$\pm$0.49 }   & 17.36\textsuperscript{$\pm$0.43 }     \\
                                   &  Oromo                                   & RougeL & 11.28\textsuperscript{$\pm$0.03 } & 10.51\textsuperscript{$\pm$0.07 } & 3.52\textsuperscript{$\pm$0.49}   & 7\textsuperscript{$\pm$1.73 }       & 14.53\textsuperscript{$\pm$0.1 }      \\
                                   &  Rundi                                   & RougeL & 19.63\textsuperscript{$\pm$0.01 } & 18.02\textsuperscript{$\pm$0.13 } & 11.82\textsuperscript{$\pm$0.39 }  & 16.13\textsuperscript{$\pm$0.03 }  & 22.57\textsuperscript{$\pm$0.04 }     \\
                                   &  Swahili                                 & RougeL & 26.38\textsuperscript{$\pm$0.02 } & 24.81\textsuperscript{$\pm$0.11 } & 15.07\textsuperscript{$\pm$0.17 }  & 21.59\textsuperscript{$\pm$0.13 }   & 29.05\textsuperscript{$\pm$0.13 }     \\
                                   &  Yoruba                                  & RougeL & 21.57\textsuperscript{$\pm$0.05 } & 20.06\textsuperscript{$\pm$0.12 } & 13.52\textsuperscript{$\pm$0.18 }  & 17.3\textsuperscript{$\pm$0.11 }    & 22.49\textsuperscript{$\pm$0.0 }     \\
                                   &  Hausa                                   & RougeL & 26.46\textsuperscript{$\pm$0.06 } & 25.76\textsuperscript{$\pm$0.02 } & 19.96\textsuperscript{$\pm$0.26 } & 25.19\textsuperscript{$\pm$0.11 }   & 30.07\textsuperscript{$\pm$0.31 }     \\
                                   &  Nigerian Pidgin                         & RougeL & 26.54\textsuperscript{$\pm$0.05 } & 25.79\textsuperscript{$\pm$0.1 }  & 14.28\textsuperscript{$\pm$1.23 }  & 20.29\textsuperscript{$\pm$0.12 }   & 27.08\textsuperscript{$\pm$0.02 }     \\
                                   &  Somali                                  & RougeL & 20.69\textsuperscript{$\pm$0.08 } & 19.21\textsuperscript{$\pm$0.06 } & 13.62\textsuperscript{$\pm$0.81 }  & 19.27\textsuperscript{$\pm$0.18 }   & 23.92\textsuperscript{$\pm$0.04 }     \\
                                   &  Tigrinya                                & RougeL & 15.84\textsuperscript{$\pm$0.13 } & 13.93\textsuperscript{$\pm$0.11 } & 6.53\textsuperscript{$\pm$0.42 }   & 10.07\textsuperscript{$\pm$0.09 }   & 16.88\textsuperscript{$\pm$0.12 }     \\ \midrule
\multirow{11}{*}{\rotatebox[origin=]{90}{\textbf{Title Generation}}}  & Multilingual                     & Bleu   & 6.53\textsuperscript{$\pm$0.02 }  & 6.65\textsuperscript{$\pm$0.08 }  & 0.1\textsuperscript{$\pm$0.02 }    & 5.2\textsuperscript{$\pm$0.02 }     & 7.52\textsuperscript{$\pm$0.07 }      \\ 
                                   & Amharic                          & Bleu   & 3.13\textsuperscript{$\pm$0.23 }  & 2.65\textsuperscript{$\pm$0.68 }  & 0.34\textsuperscript{$\pm$0.14 }   & 2.31\textsuperscript{$\pm$0.14 }    & 4.34\textsuperscript{$\pm$0.34 }      \\
                                   & Igbo                             & Bleu   & 6.95\textsuperscript{$\pm$0.13 }  & 6.9\textsuperscript{$\pm$0.22 }   & 0.77\textsuperscript{$\pm$0.12 }   & 4.61\textsuperscript{$\pm$0.14 }   & 8.47\textsuperscript{$\pm$0.07 }      \\
                                   & Oromo                            & Bleu   & 1.1\textsuperscript{$\pm$1.84 }  & 2.66\textsuperscript{$\pm$0.19 } & 0.21\textsuperscript{$\pm$0.06 }  & 1.54\textsuperscript{$\pm$0.17 }    & 3.26\textsuperscript{$\pm$0.21 }      \\
                                   & Rundi                            & Bleu   & 4.4\textsuperscript{$\pm$0.28 }   & 4.13\textsuperscript{$\pm$0.22 } & 0.84\textsuperscript{$\pm$0.07 }   & 3.33\textsuperscript{$\pm$0.23 }    & 6.05\textsuperscript{$\pm$0.5 }       \\
                                   & Swahili                          & Bleu   & 9.1\textsuperscript{$\pm$0.23 }   & 9.31\textsuperscript{$\pm$0.11 }  & 1.22\textsuperscript{$\pm$0.09 }   & 7.01\textsuperscript{$\pm$0.09 }    & 10.59\textsuperscript{$\pm$0.6 }     \\
                                   & Yoruba                           & Bleu   & 6.8\textsuperscript{$\pm$0.16 }   & 7.23\textsuperscript{$\pm$0.59 }  & 0.34\textsuperscript{$\pm$0.05}   & 5.04\textsuperscript{$\pm$2.0 }    & 7.97\textsuperscript{$\pm$0.32 }      \\
                                   & Hausa                            & Bleu   & 8.11\textsuperscript{$\pm$0.24 }  & 7.3\textsuperscript{$\pm$0.34 }   & 2.59\textsuperscript{$\pm$0.01 }   & 6.69\textsuperscript{$\pm$0.18 }    & 8.48\textsuperscript{$\pm$0.23}      \\
                                   & Nigerian Pidgin                  & Bleu   & 6.75\textsuperscript{$\pm$0.6 }   & 3.96\textsuperscript{$\pm$4.3 }  & 0.89\textsuperscript{$\pm$0.02 }   & 4.72\textsuperscript{$\pm$0.84 }    & 6.22\textsuperscript{$\pm$0.28 }      \\
                                   & Somali                           & Bleu   & 3.37\textsuperscript{$\pm$0.21 } & 3.31\textsuperscript{$\pm$0.16 }  & 0.38\textsuperscript{$\pm$0.11 }   & 2.82\textsuperscript{$\pm$0.47 }    & 5.25\textsuperscript{$\pm$0.14 }      \\
                                   & Tigrinya                         & Bleu   & 2.99\textsuperscript{$\pm$0.1 }   & 2.94\textsuperscript{$\pm$1.09 }  & 0.7\textsuperscript{$\pm$0.18 }    & 1.92\textsuperscript{$\pm$0.26 }    & 5.1\textsuperscript{$\pm$0.05 }      \\   \bottomrule
                                   {\textbf{Cloze Task}}                 & 517 Languages                                       & Bleu     & 2.36\textsuperscript{$\pm$0.11 } & 2.66\textsuperscript{$\pm$0.09 } & 0.93\textsuperscript{$\pm$0.12 } & 0.68\textsuperscript{$\pm$0.09 }   & 7.07\textsuperscript{$\pm$0.09 }    \\ 
                                   \bottomrule
                                   & \multicolumn{2}{r}{\textbf{AfroNLG Score}}                          & 12.51      & 11.05      & 5.05        & 10.85        & \textbf{31.13} \\ \bottomrule
\end{tabular}
   \caption{Performance of various models including Afri-MT5 on different datasets}
    \label{tab:results_withafri_mt5}
\end{table*}
